Dialect-robust Evaluation of Generated Text

Evaluation metrics that are not robust to dialect variation make it impossible to tell how well systems perform for many groups of users, and can even penalize systems for producing text in lower-resource dialects. However, currently, there exists no way to quantify how metrics respond to change in the dialect of a generated utterance. We thus formalize dialect robustness and dialect awareness as goals for NLG evaluation metrics. We introduce a suite of methods and corresponding statistical tests one can use to assess metrics in light of the two goals. Applying the suite to current state-of-the-art metrics, we demonstrate that they are not dialect-robust and that semantic perturbations frequently lead to smaller decreases in a metric than the introduction of dialect features. As a first step to overcome this limitation, we propose a training schema, NANO, which introduces regional and language information to the pretraining process of a metric. We demonstrate that NANO provides a size-efficient way for models to improve the dialect robustness while simultaneously improving their performance on the standard metric benchmark.

==> content/mandatory/1-ethical.tex <==
\section*{Ethical Considerations}
We hereby acknowledge that all of the co-authors of this work are aware of the provided \textit{ACL Code of Ethics} and honor the code of conduct.

Since we use pretrained language model mT5 during model pretraining and finetuning, our metric is susceptible to biased judgement with elicitation. 
While we do not explicitly address concerns around bias or sensitive content within our framework to date, we urge the interested audience to incorporate these considerations as they deploy the metric to the downstream evaluation.

The datasets used in our work, dialect features in Indian English and FRMT benchmark dataset, are all public. 
These do not contain any explicit detail that leaks information about a user's name, health, negative financial status, racial or ethnic origin, religious or philosophical affiliation, or beliefs.
